Correlations and randomness generation based on energy constraints

In a previous paper, we introduced a semi-device-independent scheme consisting of an untrusted source sending quantum states to an untrusted measuring device, with the sole assumption that the average energy of the states emitted by the source is bounded. Given this energy constraint, we showed that certain correlations between the source and the measuring device can only occur if the outcomes of the measurement are non-deterministic, i.e., these correlations certify the presence of randomness. In the present paper, we go further and show how to quantify the randomness as a function of the correlations and prove the soundness of a QRNG protocol exploiting this relation. For this purpose, we introduce (1) a semidefinite characterization of the set of quantum correlations, (2) an algorithm to lower-bound the Shannon entropy as a function of the correlations and (3) a proof of soundness using finite trials compatible with our energy assumption.

==> math_notation.tex <==
\RequirePackage{stmaryrd}
\RequirePackage{amssymb}
\RequirePackage{amsmath}
\RequirePackage{dsfont}


% Vector notation
\newcommand{\vect}[1]{\boldsymbol{#1}}
\newcommand{\sspan}{span}

% Basic
\DeclareMathOperator{\re}{Re}
\DeclareMathOperator{\im}{Im}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\DeclareMathOperator{\sgn}{sgn}

% Matrix
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\tr}{tr}
\newcommand{\id}{\mathds{1}}

% Differentials
\newcommand{\diff}[1]{\frac{\text{d}}{\text{d}#1}}
\newcommand{\pdiff}[1]{\frac{\partial}{\partial #1}}
\newcommand{\dd}{\text{d}}

% Norms
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\abs}[1]{\lvert#1\rvert}

% Dirac bra-ket notation
\newcommand{\bra}[1]{\langle#1\rvert}
\newcommand{\ket}[1]{\lvert#1\rangle}
\newcommand{\braket}[1]{\langle#1\rangle}
\newcommand{\bracket}[1]{\langle#1\rangle}

% Sets
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\bd}{bd}
\DeclareMathOperator{\extr}{extr}

% Functions
\DeclareMathOperator{\asin}{asin}
\DeclareMathOperator{\acos}{acos}
\DeclareMathOperator{\erf}{erf}

% Quantifiers
\DeclareMathOperator{\st}{subject\ to\ }
\DeclareMathOperator{\fa}{,\ for\ all\ }

% Probabilities
\DeclareMathOperator{\var}{Var}


%% Specific to the article
\newcommand{\setQ}{\mathcal{Q}}
\newcommand{\setCa}{\overline{\mathcal{C}}}
\newcommand{\vomega}{\vect{\omega}}
\newcommand{\vsigma}{\vect{\sigma}}
\newcommand{\vE}{\vect{E}}
\newcommand{\vn}{\vect{n}}
\newcommand{\vm}{\vect{m}}
\newcommand{\state}{\mathcal{S}}
\DeclareMathOperator{\E}{E}

\newcommand{\pk}{\mathrm{pk}}
\newcommand{\avg}{\mathrm{avg}}

\newcommand{\esp}[1]{\E \left[ #1 \right]}
%\newcommand{\esp}[1]{\mathbf{E}\left\llbracket #1 \right\rrbracket}
\newcommand{\Esp}[2]{\E_{#1} \left[ #2 \right]}
%\newcommand{\Esp}[2]{\mathbf{E}_{#1}\left\llbracket #2 \right\rrbracket}
\newcommand{\knuth}[1]{\llbracket #1 \rrbracket}

\DeclareMathOperator{\TV}{TV}
\DeclareMathOperator{\Pass}{Pass}


